CAST-CKT: Chaos-Aware Spatio-Temporal and Cross-City Knowledge Transfer for Traffic Flow Prediction

Traffic prediction in data-scarce, cross-city settings is challenging due to complex nonlinear dynamics and domain shifts. Existing methods often fail to capture traffic's inherent chaotic nature for effective few-shot learning. We propose CAST-CKT, a novel Chaos-Aware Spatio-Temporal and Cross-City Knowledge Transfer framework. It employs an efficient chaotic analyser to quantify traffic predictability regimes, driving several key innovations: chaos-aware attention for regime-adaptive temporal modelling; adaptive topology learning for dynamic spatial dependencies; and chaotic consistency-based cross-city alignment for knowledge transfer. The framework also provides horizon-specific predictions with uncertainty quantification. Theoretical analysis shows improved generalisation bounds. Extensive experiments on four benchmarks in cross-city few-shot settings show CAST-CKT outperforms state-of-the-art methods by significant margins in MAE and RMSE, while offering interpretable regime analysis. Code is available at https://github.com/afofanah/CAST-CKT.

==> section/related_works.tex <==
\section{Related Works}
\label{sec:related_works}

\textbf{Spatio-Temporal Forecasting and Cross-Domain Transfer.} Traffic prediction has evolved from early statistical approaches to sophisticated spatio-temporal graph neural networks that capture complex spatial dependencies and temporal dynamics \cite{li2017diffusion,zhang2021traffic,wang2025cross}, \cite{wu2020connecting}. Recent advances include attention mechanisms \cite{jiang2023spatio,huang2019diffusion}, adaptive graph learning \cite{Weng2023ADD}, and chaos-aware architectures \cite{fofanah2025chamformer}. To address data scarcity, cross-domain transfer methods employ domain adaptation \cite{Tang2022DomainAS,Li2022NetworkscaleTP}, prompt-based conditioning \cite{Hu2024PromptBasedSG,zhang2023promptst,xia2025prost}, and meta-learning frameworks \cite{Lu2022SpatioTemporalGF,Liu2023CrosscityFT}, with recent innovations in transferable graph structures \cite{Jin2023TransferableGS,yang2025cross,duan2025dynamic,li2024flashst,Rao2022FOGSFG}. However, these approaches primarily focus on spatial or statistical alignment, overlooking fundamental dynamical regime differences between urban settings.

\textbf{Chaos Theory Integration and Research Gaps.} Chaos theory provides established metrics—Lyapunov exponents, fractal dimensions, and entropy measures—for quantifying traffic predictability and nonlinear dynamics \cite{dendrinos1994traffic,shang2005chaotic,odibat2022nonlinear,fofanah2025chamformer,mcallister2024correlation}. While uncertainty quantification methods address reliability in scarce-data scenarios \cite{Qian2023towards,NOVAK2023data,qian2023uncertainty}, chaos metrics remain largely decoupled from predictive modelling. Current frameworks treat cities as statistically similar entities, failing to incorporate regime-aware adaptation based on intrinsic chaotic characteristics. This gap limits their ability to provide dynamically calibrated uncertainty estimates and robust few-shot generalisation across cities with fundamentally different predictability regimes.
